On the Local Structure of Stable Clustering Instances

We study the classic $k$-median and $k$-means clustering objectives in the beyond-worst-case scenario. We consider three well-studied notions of structured data that aim at characterizing real-world inputs: Distribution Stability (introduced by Awasthi, Blum, and Sheffet, FOCS 2010), Spectral Separability (introduced by Kumar and Kannan, FOCS 2010), Perturbation Resilience (introduced by Bilu and Linial, ICS 2010). We prove structural results showing that inputs satisfying at least one of the conditions are inherently "local". Namely, for any such input, any local optimum is close both in term of structure and in term of objective value to the global optima. As a corollary we obtain that the widely-used Local Search algorithm has strong performance guarantees for both the tasks of recovering the underlying optimal clustering and obtaining a clustering of small cost. This is a significant step toward understanding the success of local search heuristics in clustering applications.

==> preliminaries.tex <==
\subsection{Preliminaries}

\begin{defn}[$k$-Median]
  Let $p>0$ be fixed. Given a graph $G=(C\cup F, E)$ with non-negative edge weights, where the elements of $C$ are called clients and  the elements of $F$ are called centers, and a number $k$ of desired centers, the Clustering problem asks for a subset $S$ of $ F$ of cardinality at most $k$ and that minimizes
  cost$(S)= \sum_{c \in C} \min_{u \in S} \dist(c,u)$,
  where $\dist$ denotes the shortest-path distance in $G$.
\end{defn}


\begin{defn}[$k$-Means]
  Let $p>0$ be fixed. Given a graph $G=(C\cup F, E)$ with non-negative edge weights, where the elements of $C$ are called clients and  the elements of $F$ are called centers, and a number $k$ of desired centers, the Clustering problem asks for a subset $S$ of $ F$ of cardinality at most $k$ and that minimizes
  cost$(S)= \sum_{c \in C} ( \min_{u \in S} \dist(c,u))^2$,
  where $\dist$ denotes the shortest-path distance in $G$.
\end{defn}

\begin{algorithm}
  \caption{Local Search($\eps$) for $k$-Median and $k$-Means}
  \label{alg:LS}
  \begin{algorithmic}[1]
    \State \textbf{Input:} $G,k$%A graph $G = (V,E)$ with non-negative edge weights, a set $\calF\subseteq V$ of possible facility locations, a facility opening cost $f$.
    \State $S \gets$ Arbitrary subset of $\calF$.
    \While{$\exists$ $S'$ s.t. $|S'|\leq k$  \textbf{and} $|S \setminus S'| + |S' \setminus S| \leq 1/\eps$
      \textbf{and} cost($S'$) $\le$ $(1-1/n)$ cost($S$)\\}
    \State $S \gets S'$
    \EndWhile
    \State \textbf{Output:} $S$     
  \end{algorithmic}
\end{algorithm}



==> techniques.tex <==
\section{Approach and Techniques}
\label{sec:tech}

\subsection{Distribution Stability}
% As noticed by~\cite{ABS10} only a few clusters have more than a $1/\varepsilon^{-3}$ fraction 
% of the total cost of the solution. For these clusters, Local Search with appropriate neighborhood 
% size will find the optimal solution.
Assume for simplicity that all the optimal clusters cost less than an $\eps^3$ fraction of 
the total cost of the optimal solution. It results that most of the points of a cluster $C^*_i$
are contained in a small ball around $c^*_i$.
Combining this with the $\beta$-distribution-stability property, one can show that 
for any pair of centers $c^*_i,c^*_j$, the points contained in a small ball around $c^*_i$ 
are far from the points contained in small ball around $c^*_j$.
Thus, because of the objective function, the local search algorithm 
has a strong incentive to dedicate exactly one center for most of the clusters of the optimal solution. 
In addition, we can show that for most of these ``good'' centers
the corresponding cluster in the local solution is very similar to the optimal cluster
(see Figure~\ref{fig:local}). In total, only very few clusters (a function of $\eps$ and $\beta$)
of the optimal solution are not present in the local solution. We then conlude our proof using local optimality.

Our proof includes a few ingredients from~\cite{ABS10} such as the notion of \emph{inner-ring} (we work with a slightly
more general definition) and distinguishing between \emph{cheap} and \emph{expensive} clusters. However, our 
analysis is slightly stronger as it allows us to analyze not only the cost of the solution of the algorithm, but also
the structure of its clusters.

Euclidean inputs can be straightforwardly ``discretized'' by computing an appropriate candidate set of centers,
for instance via Matousek's approximate centroid set~\cite{Mat00}.

\subsection{Perturbation Resilience}
The tight approximation factor of $3+\varepsilon$ of Local Search for $k$-median implies a locality 
gap\footnote{The locality gap is the maximum ratio between a local optimum and a global optimum.} of $3$.
The main lemma shows that perturbation resilience implies that locally optimal solutions 
for a local neighborhood of appropriate size are equal to the global optimum.
We then provide a careful analysis of $1/\eps$-locally-optimal solutions.
% Since Local Search converges in a locally optimal solution, it then also finds the global optimum.

\subsection{Spectral Separability}
In Section~\ref{sec:euclid} we study the spectral separability conditions for the Euclidean $k$-means problem.

Nowadays, a standard preprocessing step in Euclidean $k$-means clustering is to project onto the subspace spanned by the rank $k$-approximation.
Indeed, this is the first step of the algorithm by Kumar and Kannan~\cite{KuK10} (see Algorithm~\ref{alg:specmeans}).
\begin{algorithm}
  \caption{$k$-means with spectral initialization~\cite{KuK10}}
  \label{alg:kmeanspec}
  \begin{algorithmic}[1]
%    \State {\textbf{Input:} $A,k$}
    \State{Project points onto the best rank $k$ subspace}
    \State{Compute a clustering $C$ with constant approximation factor on the projection}
    \State{Initialize centroids of each cluster of $C$ as centers in the original space} 
    \State{Run Lloyd's $k$-means until convergence}
  \end{algorithmic}
    \label{alg:specmeans}
\end{algorithm}

In general, projecting onto the best rank $k$ subspace and computing a constant approximation on the projection results in a constant approximation
in the original space.
Kumar and Kannan~\cite{KuK10} and later Awasthi and Sheffet~\cite{AwS12} gave tighter bounds if the spectral separation is large enough. 
%that the separation condition $\frac{OPT_k}{OPT_{k-1}}\leq \varepsilon$ by Ostrovsky et al.~\cite{ORSS12} implies the proximity condition with $\beta=\Omega(k)$ for all but an $\varepsilon$ fraction of the points and hence also the spectral separation condition.
%In this case, the algorithm~\ref{alg:specmeans} is a PTAS.
%Moreover, the solution computed after step $2$ is already shown to be a $(1+O(\sqrt{k\varepsilon}))$-approximation, which was later improved by Awasthi and Sheffet~\cite{AwS12} to $(1+O(\sqrt{\varepsilon}))$.
Our algorithm omits steps 3 and 4.
Instead, we project onto slightly more dimensions and subsequently use Local Search as the constant factor approximation in step 2.
To utilize Local Search, we further require a candidate set of solutions, which is described in Section~\ref{sec:euclidperturb}.
For pseudocode, we refer to Algorithm~\ref{alg:specls}.

It is easy to show that spectral separability implies distribution stability if the dimension is of order $k$: (1) the distance between centers is $$\Omega(\left(\frac{1}{\sqrt{|C_i^*|}}+\frac{1}{\sqrt{|C_j^*|}}\right) k\cdot ||A-C||_2) = \Omega\left(\left(\frac{1}{\sqrt{|C_i^*|}}+\frac{1}{\sqrt{|C_j^*|}}\right)\sqrt{\opt}\right),$$ and (2) the distance of any point to the ``wrong'' center is at least $1/2$ of this amount, i.e. the cost of assigning a point to the ``wrong'' cluster is $\Omega(\frac{\opt}{|C_j|})$.
Projecting onto sufficiently many dimensions allows us to transform a high dimensional point set into a low dimensional one, see for instance recent work by Cohen et al.~\cite{CfLocalEMMP15}.
The projection retains the cost and spectral separability of a clustering, however it does not preserve optimality.
In particular, the distance of a single point to the centroids of the clusters can be arbitrarily distorted (see Figure~\ref{fig:spec}), which prevents us from using the naive reduction to distribution stability.

Instead, we locally improve on the optimal clustering by reassigning points (Lemma~\ref{lem:mainspec}).
A large contraction of relevant distances can only happen for few points, i.e. the cluster sizes are roughly the same.
For the remaining points, we can show that they are guaranteed to have a minimum distance to the wrong center.


%Note that the while we can omit step 2 of the algorithm if $k<\log n$, it seems necessary to execute both projections in this order if $\log n < k$.
%%\begin{algorithm}
%%  \caption{Project and Local Search}
%%  \begin{algorithmic}[1]
%%%    \State {\textbf{Input:} $A,k$}
%%    \State{Project points $A$ onto the best rank $3k/\varepsilon$ subspace}
%%    \State{Embed points into a random subspace of dimension $O(\varepsilon^{-2}\log n)$}
%%    \State{Compute candidate centers (Lemma~\ref{lem:discrete}}
%%    \State{Local Search($\varepsilon^{-4}/(\alpha-3)^2$)}
%%   	\State{Output clustering with centroids computed from $A$}
%%  \end{algorithmic}
%%    \label{alg:specls}
%%\end{algorithm}
%
%%For the first step of the algorithm, we will utilize a recent result stating that any point set $A$ can be projected into a low-dimensional space which forms a point set $A_m$ while retaining the cost of any $k$-means clustering. 
%%We show that spectral separability with $\gamma \in \Omega(\sqrt{k})$ of $A$ further implies the existence of a sufficiently good clustering with constant distribution stability in $A_m$.
%%For the second step, we show that centroids are preserved under Johnson-Lindenstrauss-type embeddings.
%%We would like to note that the sequential application of these embeddings seems to be necessary.
%%The third step requires from us the generation of a candidate set of centers that preserve both cost, as well as perturbations stability.
%
%The correctness of Algorithm~\ref{alg:specls} (and Theorem~\ref{thm:spectralptas}) will be proven in two main parts. 
%The first part (Section~\ref{sec:spectral}) relates spectral stability and distribution stability.
%We will show that there exists a clustering $C'$ not necessarily equal to $C$ using the projection of $S$ onto the best low rank approximation $A_m$, such that $C'$ with centers $S$ has constant distribution stability.
%Technically, we combine parts of the analysis of Kumar and Kannan~\cite{KuK10} and Awasthi and Sheffet~\cite{AwS12} with recent results on cost-preserving low-rank projections of Cohen et al.~\cite{CEMMP15}.
%
%The second part (Section~\ref{sec:euclidperturb}) will deal with the generation of candidate solutions with little dependency on the dimension.
%Indeed, there exist many constructions for a small set of candidate centers with good cost (see Feldman and Langberg~\cite{FeL11} and references therein).
%However, these constructions do not seem to preserve distribution stability as well\footnote{Matousek's approximate centroid sets~\cite{Mat00} can be shown to preserve distribution stability, if the centers of the clusters are restricted to centroids.}.
%Instead, we utilize known results on construction $\varepsilon$-nets in Euclidean spaces.
%This construction is exponential in $d$ (resp. $k$ after executing step 1 of Algorithm~\ref{alg:specls}).
%To avoid this dependency, we apply a random linear, near isometric embedding of target dimension $O(\varepsilon^{-2}\log n)$.
%It is well known, that these embeddings preserve pairwise distances, and it is not too difficult to show that they preserve distribution stability as well.

